Accelerated First Order Methods for Variational Imaging

In this thesis, we offer a thorough investigation of different regularisation terms used in variational imaging problems, together with detailed optimisation processes of these problems. We begin by studying smooth problems and partially non-smooth problems in the form of Tikhonov denoising and Total Variation (TV) denoising, respectively. For Tikhonov denoising, we study an accelerated gradient method with adaptive restart, which shows a very rapid convergence rate. However, it is not straightforward to apply this fast algorithm to TV denoising, due to the non-smoothness of its built-in regularisation. To tackle this issue, we propose to utilise duality to convert such a non-smooth problem into a smooth one so that the accelerated gradient method with restart applies naturally. However, we notice that both Tikhonov and TV regularisations have drawbacks, in the form of blurred image edges and staircase artefacts, respectively. To overcome these drawbacks, we propose a novel adaption to Total Generalised Variation (TGV) regularisation called Total Smooth Variation (TSV), which retains edges and meanwhile does not produce results which contain staircase artefacts. To optimise TSV effectively, we then propose the Accelerated Proximal Gradient Algorithm (APGA) which also utilises adaptive restart techniques. Compared to existing state-of-the-art regularisations (e.g. TV), TSV is shown to obtain more effective results on denoising problems as well as advanced imaging applications such as magnetic resonance imaging (MRI) reconstruction and optical flow. TSV removes the staircase artefacts observed when using TV regularisation, but has the added advantage over TGV that it can be efficiently optimised using gradient based methods with Nesterov acceleration and adaptive restart. Code is available at https://github.com/Jbartlett6/Accelerated-First-Order-Method-for-Variational-Imaging.

==> jose/preamble.tex <==
%---------------------------------------------------------%
%------------------ Document Preamble --------------------%
%---------------------------------------------------------%

%-------------------------------------------%
%---- First load the necessary packages ----%
%-------------------------------------------%


\usepackage{amsmath}  % Improves typographic quality of mathematical output.
\usepackage{amsfonts} % For mathematical fonts.
\usepackage{cleveref}
% Package for no indentation and to include a line between paragraphs.
\usepackage[parfill]{parskip}

% Set the layout of the document.

\usepackage{subfigure}
\usepackage{amsmath}
\usepackage[algo2e,ruled]{algorithm2e}
\usepackage{amsthm} % Needed to typeset theorem environments.
\usepackage[affil-it]{authblk} % Needed for author and affiliation.
\usepackage{amsopn} % Allows the declaration of new mathematical operators.
\usepackage{amssymb} % Extended set of mathematical symbols.
\usepackage{mathrsfs} % Raph Smith's mathematical script font.
\usepackage{booktabs} % Improves the typographical quality of tables.
\usepackage{natbib} % Citations and bibliography.
\usepackage{tikz} % Extends the figure generation capabilities of LaTeX.
\usepackage{algorithm} % Necessary for including algorithmic structures.
\usepackage{float} % Allows the creation of own floating environments.
\usepackage{caption} % Allows the customisation of captions.
\usepackage{abstract} % For including abstracts in documents.
\usepackage{listings} % For the inclusion of source code.
\usepackage{color} % Used for colour commands.

% Automatic inclusion of hyperlinks with back references.
%\usepackage[pagebackref]{hyperref} 

%-------------------------------------------%

% Making a float for an algorithm.
\newfloat{algorithm}{t}{lop}
\renewcommand{\thealgorithm}{\arabic{section}.\arabic{algorithm}} 

% Numbers equations by section.
\numberwithin{equation}{section}

% Set biliography style.
\bibliographystyle{apalike}

% Commands for special set of numbers.
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\EE}{\mathbb{E}}

% Commands for useful operators.
\newcommand{\di}{\text{diag}}
\newcommand{\de}{\mathrm{d}}
\newcommand{\si}{\Sigma}
\newcommand{\del}{\Delta}
\newcommand{\cov}[1]{\, {\rm cov}\left( #1 \right) }
\newcommand{\var}[1]{\, {\rm var}\left( #1 \right) }
\newcommand{\toas}{\xrightarrow{\text{a.s.}}}
\newcommand{\todis}{\xrightarrow{\text{d}}}
\newcommand{\supp}{\text{supp}}
\newcommand{\doubint}{\!\int\!\!\!\int}

% Command for text within a math sub/super-script.
\newcommand{\stext}[1]{\text{\scriptsize{#1}}}

% Theorem definitions/
\newtheorem{lemma}{Lemma}[section]
\newtheorem{theorem}[lemma]{Theorem}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{corollary}[lemma]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]

\theoremstyle{remark}
\newtheorem{remark}{Remark}[section]
\newtheorem{example}[remark]{Example}

% An environment for centre aligning equations which extend past the text width.
\newenvironment{longeq}
 {\begin{displaymath}\begin{lrbox}{\overlongequation}$\displaystyle}
 {$\end{lrbox}\makebox[0pt]{\usebox{\overlongequation}}\end{displaymath}}

% Listings options.

\lstset{ %
basicstyle=\footnotesize,       % the size of the fonts that are used for the code
backgroundcolor=\color{white},  % choose the background color. You must add \usepackage{color}
showspaces=false,               % show spaces adding particular underscores
showstringspaces=false,         % underline spaces within strings
showtabs=false,                 % show tabs within strings adding particular underscores
frame=single,           % adds a frame around the code
tabsize=2,          % sets default tabsize to 2 spaces
captionpos=b,           % sets the caption-position to bottom
breaklines=true,        % sets automatic line breaking
breakatwhitespace=false,    % sets if automatic breaks should only happen at whitespace
escapeinside={\%*}{*)}          % if you want to add a comment within your code
}

